Dual Box Embeddings for the Description Logic EL++

OWL ontologies, whose formal semantics are rooted in Description Logic (DL), have been widely used for knowledge representation. Similar to Knowledge Graphs (KGs), ontologies are often incomplete, and maintaining and constructing them has proved challenging. While classical deductive reasoning algorithms use the precise formal semantics of an ontology to predict missing facts, recent years have witnessed growing interest in inductive reasoning techniques that can derive probable facts from an ontology. Similar to KGs, a promising approach is to learn ontology embeddings in a latent vector space, while additionally ensuring they adhere to the semantics of the underlying DL. While a variety of approaches have been proposed, current ontology embedding methods suffer from several shortcomings, especially that they all fail to faithfully model one-to-many, many-to-one, and many-to-many relations and role inclusion axioms. To address this problem and improve ontology completion performance, we propose a novel ontology embedding method named Box$^2$EL for the DL EL++, which represents both concepts and roles as boxes (i.e., axis-aligned hyperrectangles), and models inter-concept relationships using a bumping mechanism. We theoretically prove the soundness of Box$^2$EL and conduct an extensive experimental evaluation, achieving state-of-the-art results across a variety of datasets on the tasks of subsumption prediction, role assertion prediction, and approximating deductive reasoning.

==> tables/anatomy_prediction.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[h]
    \centering
    \caption{Detailed subsumption prediction results on Anatomy.}
    \label{tab:anatomy}
    \begin{tabular}{@{}llrrrrrrr@{}}
        \toprule
        & Model    & H@1        & H@10       & H@100      & Med          & MRR           & MR            & AUC           \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF1}}      & ELEm     & 0.07 & 0.30 & 0.57          & 43           & 0.14 & 9059          & 0.91          \\
        & \emelpp & \textbf{0.08} & 0.29 & 0.53 & 60 & 0.14 & 10414 & 0.90\\\
        & BoxEL & 0.01 & 0.05 & 0.16 & 1828 & 0.03 & 9597 & 0.91\\
        & ELBE     & 0.05          & 0.24          & 0.55          & 68           & 0.11          & 5177          & 0.95          \\
        & \boxsqel & 0.07          & \textbf{0.34}          & \textbf{0.65} & \textbf{27}  & \textbf{0.15}          & \textbf{2894} & \textbf{0.97} \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF2}}      & ELEm     & 0.03          & 0.18          & 0.42          & 394          & 0.08          & 11592         & 0.89          \\
        & \emelpp & 0.03 & 0.18 & 0.35 & 1291 & 0.08 & 15759 & 0.85\\
        & BoxEL & 0.00 & 0.00 & 0.00 & 17607 & 0.00 & 26872 & 0.75\\
        & ELBE     & 0.02          & 0.11          & 0.26          & 1394         & 0.05          & 4885          & 0.96          \\
        & \boxsqel & \textbf{0.16} & \textbf{0.41} & \textbf{0.64} & \textbf{26}  & \textbf{0.24} & \textbf{1928} & \textbf{0.98} \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF3}}      & ELEm     & 0.12          & 0.47          & 0.69          & 13           & 0.23          & 4686          & 0.96          \\
        & \emelpp & 0.13 & 0.42 & 0.60 & 23 & 0.23 & 7097 & 0.93\\
        & BoxEL & 0.04 & 0.17 & 0.36 & 567 & 0.08 & 11095 & 0.90\\
        & ELBE     & 0.04          & 0.44          & 0.70          & 16           & 0.18          & 5408          & 0.95          \\
        & \boxsqel & \textbf{0.21} & \textbf{0.56} & \textbf{0.75} & \textbf{7}   & \textbf{0.33} & \textbf{2466} & \textbf{0.98} \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF4}}      & ELEm     & 0.00          & 0.03          & \textbf{0.23}          & \textbf{813}          & \textbf{0.01}          & 10230         & 0.91          \\
        & \emelpp & 0.00 & 0.02 & 0.17 & 1470 & \textbf{0.01} & 10951 & 0.90\\
        & BoxEL & 0.00 & 0.00 & 0.00 & 38942 & 0.00 & 41283 & 0.61\\
        & ELBE     & 0.00          & 0.02          & 0.06          & 6261         & \textbf{0.01}          & 15187         & 0.86          \\
        & \boxsqel & 0.00          & \textbf{0.05} & 0.14 & 3065 & \textbf{0.01} & \textbf{8366} & \textbf{0.92} \\ \bottomrule
    \end{tabular}
\end{table*}

==> tables/both.tex <==
\begin{table*}[t]
    %\begin{minipage}{\textwidth}
     %   \centering


    %\end{minipage}
    \begin{minipage}{0.49\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{@{}llrrrrrrr@{}}
            \toprule
            Dataset                  & Model & Hits@1 & Hits@10       & Hits@100 & Med  & MRR  & MR   & AUC  \\ \midrule
            \multirow{3}{*}{GALEN}   & ELEm  & 0.01   & 0.12          & 0.29     & 1662 & 0.05 & 5153 & 0.78 \\
            & ELBE  & 0.02   & 0.14          & 0.27     & 1865 & 0.06 & 5303 & 0.77 \\
            & \boxsqel & \textbf{0.04} & \textbf{0.18} & \textbf{0.36} & \textbf{643} & \textbf{0.09} & \textbf{4511} & \textbf{0.81} \\ \midrule
            \multirow{3}{*}{GO}      & ELEm  & 0.03   & \textbf{0.24} & 0.43     & 272  & 0.09 & 6204 & 0.86 \\
            & ELBE  & 0.01   & 0.10          & 0.22     & 1838 & 0.04 & 6986 & 0.85 \\
            & \boxsqel & \textbf{0.04} & 0.23          & \textbf{0.60} & \textbf{50}  & \textbf{0.10} & \textbf{3151} & \textbf{0.93} \\ \midrule
            \multirow{3}{*}{Anatomy} & ELEm  & 0.10   & 0.40          & 0.64     & 22   & 0.19 & 6464 & 0.94 \\
            & ELBE  & 0.04   & 0.36          & 0.63     & 29   & 0.15 & 5400 & 0.95 \\
            & \boxsqel & \textbf{0.19} & \textbf{0.48} & \textbf{0.69} & \textbf{13}  & \textbf{0.29} & \textbf{3312} & \textbf{0.97} \\ \bottomrule
        \end{tabular}%
        }
        \caption{Subsumption prediction results combined across normal forms.}
        \label{tab:combined}
    \end{minipage}

    \begin{minipage}{0.49\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{@{}llrrrrrrr@{}}
            \toprule
            Normal form               & Model    & Hits@1        & Hits@10       & Hits@100      & Med           & MRR           & MR            & AUC           \\ \midrule
            \multirow{3}{*}{NF1}      & ELEm     & 0.01          & 0.16          & 0.40          & 430           & 0.06          & 3568          & 0.85          \\
            & ELBE     & \textbf{0.03} & 0.24          & 0.47          & 138           & \textbf{0.10} & 2444          & 0.89          \\
            & \boxsqel & 0.02          & \textbf{0.25} & \textbf{0.55} & \textbf{62}   & 0.09          & \textbf{2039} & \textbf{0.91} \\ \midrule
            \multirow{3}{*}{NF2}      & ELEm     & 0.01          & 0.07          & 0.17          & 5106          & 0.03          & 7432          & 0.68          \\
            & ELBE     & 0.03          & 0.06          & 0.11          & 6476          & 0.04          & 8068          & 0.65          \\
            & \boxsqel & \textbf{0.05} & \textbf{0.13} & \textbf{0.22} & \textbf{3468} & \textbf{0.08} & \textbf{7246} & \textbf{0.69} \\ \midrule
            \multirow{3}{*}{NF3}      & ELEm     & 0.02          & 0.14          & 0.28          & 1479          & 0.05          & 4831          & 0.79          \\
            & ELBE     & 0.03          & 0.14          & 0.25          & 2154          & 0.07          & 5072          & 0.78          \\
            & \boxsqel & \textbf{0.08} & \textbf{0.19} & \textbf{0.31} & \textbf{1060} & \textbf{0.12} & \textbf{4530} & \textbf{0.80} \\ \midrule
            \multirow{3}{*}{NF4}      & ELEm     & 0.00          & 0.05          & 0.18          & 3855          & \textbf{0.02} & \textbf{6793} & \textbf{0.71} \\
            & ELBE     & 0.00          & 0.03          & 0.07          & 7563          & 0.01          & 8884          & 0.62          \\
            & \boxsqel & 0.00          & \textbf{0.08} & \textbf{0.19} & \textbf{3426} & \textbf{0.02} & 6806          & \textbf{0.71} \\ \bottomrule
        \end{tabular}%
        }
        \caption{Detailed subsumption prediction results on GALEN.}
        \label{tab:galen}
    \end{minipage}
\end{table*}

==> tables/bumps_reg.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}lrrrrrrr@{}}
        \toprule
        Model       & H@1        & H@10       & H@100      & Med          & MRR           & MR            & AUC           \\ \midrule
        \boxsqel-NB & 0.00          & 0.03          & 0.12          & 7336         & 0.01          & 8673          & 0.63          \\
        \boxsqel-NR & \textbf{0.04} & 0.16          & 0.33          & 877          & 0.08          & 4789          & 0.79          \\
        \boxsqel    & \textbf{0.04} & \textbf{0.18} & \textbf{0.36} & \textbf{643} & \textbf{0.09} & \textbf{4511} & \textbf{0.81} \\ \bottomrule
    \end{tabular}%
    }
    \caption{Impact of bump vectors and regularisation on the performance of \boxsqel\@. We compare our model with a version without bump vectors (\boxsqel-NB) and a version without regularization (\boxsqel-NR).}
    \label{tab:bumps_reg}
\end{table}

==> tables/combined.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
    \centering
    \caption{Subsumption prediction results combined across normal forms.}
    \label{tab:combined}
    \begin{tabular}{@{}llrrrrrrr@{}}
        \toprule
                          & Model & H@1 & H@10       & H@100 & Med  & MRR  & MR   & AUC  \\ \midrule
        \multirow{4}{*}{\rotatebox[origin=c]{90}{GALEN}}   & ELEm  & 0.01   & 0.12          & 0.29     & 1662 & 0.05 & 5153 & 0.78 \\
        & \emelpp  & 0.01   & 0.11          & 0.24     & 2295 & 0.05 & 5486 & 0.76\\
        & ELBE  & 0.02   & 0.14          & 0.27     & 1865 & 0.06 & 5303 & 0.77 \\
        & \boxsqel & \textbf{0.04} & \textbf{0.18} & \textbf{0.36} & \textbf{643} & \textbf{0.09} & \textbf{4511} & \textbf{0.81} \\ \midrule
        \multirow{4}{*}{\rotatebox[origin=c]{90}{GO}}      & ELEm  & 0.03   & \textbf{0.24} & 0.43     & 272  & 0.09 & 6204 & 0.86 \\
        & \emelpp  & 0.03   & 0.23          & 0.38     & 597 & 0.09 & 6710 & 0.85\\
        & ELBE  & 0.01   & 0.10          & 0.22     & 1838 & 0.04 & 6986 & 0.85 \\
        & \boxsqel & \textbf{0.04} & 0.23          & \textbf{0.60} & \textbf{50}  & \textbf{0.10} & \textbf{3151} & \textbf{0.93} \\ \midrule
        \multirow{4}{*}{\rotatebox[origin=c]{90}{Anatomy}} & ELEm  & 0.10   & 0.40          & 0.64     & 22   & 0.19 & 6464 & 0.94 \\
        & \emelpp  & 0.11   & 0.36          & 0.57     & 36 & 0.19 & 8472 & 0.92\\
        & ELBE  & 0.04   & 0.36          & 0.63     & 29   & 0.15 & 5400 & 0.95 \\
        & \boxsqel & \textbf{0.19} & \textbf{0.48} & \textbf{0.69} & \textbf{13}  & \textbf{0.29} & \textbf{3312} & \textbf{0.97} \\ \bottomrule
    \end{tabular}%
\end{table}

==> tables/detailed.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
    \centering
    \caption{Detailed subsumption prediction results on GO (a) and Anatomy~(b).}
    \label{tab:detailed}
    \begin{subtable}[t]{0.48\linewidth}
        \centering
        \caption{}
        \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}llrrrrrrr@{}}
        \toprule
                       & Model    & H@1 & H@10       & H@100      & Med  & MRR  & MR            & AUC           \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF1}}      & ELEm     & 0.01   & 0.13          & 0.35          & 590  & 0.05 & 6433          & 0.86          \\
        & \emelpp & 0.01 & 0.12 & 0.30 & 1023 & 0.05 & 6709 & 0.85\\
        & BoxEL     & 0.00 & 0.01 & 0.05 & 5374 & 0.00 & 13413 & 0.71        \\
        & ELBE     & 0.01   & 0.10          & 0.24          & 1156 & 0.04 & 5657          & 0.88          \\
        & \boxsqel & \textbf{0.03} & \textbf{0.17} & \textbf{0.58} & \textbf{58} & \textbf{0.08} & \textbf{2686} & \textbf{0.94} \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF2}}      & ELEm     & 0.12   & 0.49          & 0.63          & 11   & 0.24 & 4508          & 0.90          \\
        & \emelpp & 0.11 & 0.44 & 0.55 & 23 & 0.21 & 5169 & 0.89\\
        & BoxEL & 0.00 & 0.00 & 0.00 & 22882 & 0.00 & 23007 & 0.50\\
        & ELBE     & 0.01   & 0.05          & 0.09          & 6456 & 0.02 & 9421          & 0.80          \\
        & \boxsqel & \textbf{0.18} & \textbf{0.58} & \textbf{0.75} & \textbf{6}  & \textbf{0.31} & \textbf{2104} & \textbf{0.95} \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF3}} & ELEm     & \textbf{0.06} & \textbf{0.40} & 0.52 & \textbf{54} & \textbf{0.15} & 6292          & 0.86          \\
        & \emelpp & 0.05 & 0.39 & 0.48 & 210 & \textbf{0.15} & 7788 & 0.83\\
        & BoxEL & 0.00 & 0.00 & 0.00 & 17027 & 0.00 & 18947 & 0.59\\
        & ELBE     & 0.02   & 0.15          & 0.30          & 959  & 0.07 & 7131          & 0.84          \\
        & \boxsqel & 0.00   & 0.18          & \textbf{0.53}          & 79   & 0.05 & \textbf{5042} & \textbf{0.89} \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF4}} & ELEm     & 0.01 & 0.49 & 0.60          & \textbf{12} & 0.12 & 6272          & 0.86          \\
        & \emelpp & 0.01 & 0.49 & 0.58 & \textbf{12} & 0.13 & 6442 & 0.86\\
        & BoxEL & \textbf{0.09} & \textbf{0.54} & 0.54 & 2215 & \textbf{0.28} & 9673 & 0.79\\
        & ELBE     & 0.00   & 0.07          & 0.12          & 9049 & 0.02 & 12868         & 0.72          \\
        & \boxsqel & 0.00   & 0.37          & \textbf{0.64} & 20   & 0.08 & \textbf{4989} & \textbf{0.89} \\ \bottomrule
    \end{tabular}%
        }%
    \end{subtable}
    \hfill
    \begin{subtable}[t]{0.48\linewidth}
        \centering
        \caption{}
        \resizebox{\linewidth}{!}{
            \begin{tabular}{@{}llrrrrrrr@{}}
        \toprule
        & Model    & H@1        & H@10       & H@100      & Med          & MRR           & MR            & AUC           \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF1}}      & ELEm     & 0.07 & 0.30 & 0.57          & 43           & 0.14 & 9059          & 0.91          \\
        & \emelpp & \textbf{0.08} & 0.29 & 0.53 & 60 & 0.14 & 10414 & 0.90\\\
        & BoxEL & 0.01 & 0.05 & 0.16 & 1828 & 0.03 & 9597 & 0.91\\
        & ELBE     & 0.05          & 0.24          & 0.55          & 68           & 0.11          & 5177          & 0.95          \\
        & \boxsqel & 0.07          & \textbf{0.34}          & \textbf{0.65} & \textbf{27}  & \textbf{0.15}          & \textbf{2894} & \textbf{0.97} \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF2}}      & ELEm     & 0.03          & 0.18          & 0.42          & 394          & 0.08          & 11592         & 0.89          \\
        & \emelpp & 0.03 & 0.18 & 0.35 & 1291 & 0.08 & 15759 & 0.85\\
        & BoxEL & 0.00 & 0.00 & 0.00 & 17607 & 0.00 & 26872 & 0.75\\
        & ELBE     & 0.02          & 0.11          & 0.26          & 1394         & 0.05          & 4885          & 0.96          \\
        & \boxsqel & \textbf{0.16} & \textbf{0.41} & \textbf{0.64} & \textbf{26}  & \textbf{0.24} & \textbf{1928} & \textbf{0.98} \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF3}}      & ELEm     & 0.12          & 0.47          & 0.69          & 13           & 0.23          & 4686          & 0.96          \\
        & \emelpp & 0.13 & 0.42 & 0.60 & 23 & 0.23 & 7097 & 0.93\\
        & BoxEL & 0.04 & 0.17 & 0.36 & 567 & 0.08 & 11095 & 0.90\\
        & ELBE     & 0.04          & 0.44          & 0.70          & 16           & 0.18          & 5408          & 0.95          \\
        & \boxsqel & \textbf{0.21} & \textbf{0.56} & \textbf{0.75} & \textbf{7}   & \textbf{0.33} & \textbf{2466} & \textbf{0.98} \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF4}}      & ELEm     & 0.00          & 0.03          & \textbf{0.23}          & \textbf{813}          & \textbf{0.01}          & 10230         & 0.91          \\
        & \emelpp & 0.00 & 0.02 & 0.17 & 1470 & \textbf{0.01} & 10951 & 0.90\\
        & BoxEL & 0.00 & 0.00 & 0.00 & 38942 & 0.00 & 41283 & 0.61\\
        & ELBE     & 0.00          & 0.02          & 0.06          & 6261         & \textbf{0.01}          & 15187         & 0.86          \\
        & \boxsqel & 0.00          & \textbf{0.05} & 0.14 & 3065 & \textbf{0.01} & \textbf{8366} & \textbf{0.92} \\ \bottomrule
    \end{tabular}%
        }%
    \end{subtable}%
\end{table*}

==> tables/emelpp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}
    \centering
        \begin{tabular}{@{}llrrrrrr@{}}
            \toprule
            Dataset                           & Model           & Hits@1        & Hits@10       & Hits@100      & Med         & MR            & AUC           \\ \midrule
            \multirow{5}{*}{\textsf{GALEN}}   & ELEm            & 0.01          & 0.08          & 0.15          & 6658        & 8321          & 0.64          \\
            & EmEL\texttt{++} & 0.02          & 0.11          & 0.17          & 6623        & 8407          & 0.65          \\
            & BoxEL           & --            & 0.12          & 0.23          & --          & 2922          & 0.89          \\
            & ELBE            & \textbf{0.04} & 0.27          & 0.52          & 84          & \textbf{2104} & \textbf{0.91} \\
            & \boxsqel        & \textbf{0.04} & \textbf{0.32} & \textbf{0.56} & \textbf{52} & 2166          & \textbf{0.91} \\ \midrule
            \multirow{5}{*}{\textsf{GO}}      & ELEm            & 0.01          & 0.09          & 0.23          & 4302        & 13719         & 0.73          \\
            & EmEL\texttt{++} & 0.01          & 0.10          & 0.24          & 2908        & 11050         & 0.78          \\
            & BoxEL           & --            & 0.09          & 0.24          & --          & 8010          & 0.83          \\
            & ELBE            & 0.02          & 0.12          & 0.27          & 865         & 5458          & 0.88          \\
            & \boxsqel        & \textbf{0.03} & \textbf{0.16} & \textbf{0.54} & \textbf{76} & \textbf{3670} & \textbf{0.92} \\ \midrule
            \multirow{5}{*}{\textsf{ANATOMY}} & ELEm            & 0.04          & 0.19          & 0.41          & 640         & 28564         & 0.73          \\
            & EmEL\texttt{++} & 0.04          & 0.18          & 0.40          & 381         & 24421         & 0.76          \\
            & BoxEL           & --            & 0.19          & 0.43          & --          & 8688          & 0.92          \\
            & ELBE            & 0.05          & 0.20          & 0.46          & 159         & 12850         & 0.88          \\
            & \boxsqel        & \textbf{0.06} & \textbf{0.29} & \textbf{0.52} & \textbf{75} & \textbf{7265} & \textbf{0.93} \\ \bottomrule
        \end{tabular}%
    \caption{Test caption}
    \label{tab:test}
\end{table}

==> tables/galen_prediction.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
    \centering
    \caption{Detailed subsumption prediction results on GALEN.}
    \label{tab:galen}
    \begin{tabular}{@{}llrrrrrrr@{}}
        \toprule
                       & Model    & H@1        & H@10       & H@100      & Med           & MRR           & MR            & AUC           \\ \midrule
        \multirow{4}{*}{\rotatebox{90}{NF1}}      & ELEm     & 0.01          & 0.16          & 0.40          & 430           & 0.06          & 3568          & 0.85          \\
        & \emelpp     & 0.02 & 0.16          & 0.37          & 632           & 0.06 & 3765          & 0.84          \\
        & ELBE     & \textbf{0.03} & 0.24          & 0.47          & 138           & \textbf{0.10} & 2444          & 0.89          \\
        & \boxsqel & 0.02          & \textbf{0.25} & \textbf{0.55} & \textbf{62}   & 0.09          & \textbf{2039} & \textbf{0.91} \\ \midrule
        \multirow{4}{*}{\rotatebox{90}{NF2}}      & ELEm     & 0.01          & 0.07          & 0.17          & 5106          & 0.03          & 7432          & 0.68          \\
        & \emelpp & 0.01 & 0.07 & 0.15 & 5750 & 0.03 & 7767 & 0.66\\
        & ELBE     & 0.03          & 0.06          & 0.11          & 6476          & 0.04          & 8068          & 0.65          \\
        & \boxsqel & \textbf{0.05} & \textbf{0.13} & \textbf{0.22} & \textbf{3468} & \textbf{0.08} & \textbf{7246} & \textbf{0.69} \\ \midrule
        \multirow{4}{*}{\rotatebox{90}{NF3}}      & ELEm     & 0.02          & 0.14          & 0.28          & 1479          & 0.05          & 4831          & 0.79          \\
        & \emelpp & 0.02 & 0.11 & 0.22 & 2240 & 0.05 & 5348 & 0.77\\
        & ELBE     & 0.03          & 0.14          & 0.25          & 2154          & 0.07          & 5072          & 0.78          \\
        & \boxsqel & \textbf{0.08} & \textbf{0.19} & \textbf{0.31} & \textbf{1060} & \textbf{0.12} & \textbf{4530} & \textbf{0.80} \\ \midrule
        \multirow{4}{*}{\rotatebox{90}{NF4}}      & ELEm     & 0.00          & 0.05          & 0.18          & 3855          & \textbf{0.02} & \textbf{6793} & \textbf{0.71} \\
        & \emelpp & 0.00 & 0.04 & 0.12 & 4458 & 0.01 & 7020 & 0.70\\
        & ELBE     & 0.00          & 0.03          & 0.07          & 7563          & 0.01          & 8884          & 0.62          \\
        & \boxsqel & 0.00          & \textbf{0.08} & \textbf{0.19} & \textbf{3426} & \textbf{0.02} & 6806          & \textbf{0.71} \\ \bottomrule
    \end{tabular}%
\end{table}

==> tables/go_prediction.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
    \centering
    \caption{Detailed subsumption prediction results on GO\@.}
    \label{tab:go}
    \begin{tabular}{@{}llrrrrrrr@{}}
        \toprule
                       & Model    & H@1 & H@10       & H@100      & Med  & MRR  & MR            & AUC           \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF1}}      & ELEm     & 0.01   & 0.13          & 0.35          & 590  & 0.05 & 6433          & 0.86          \\
        & \emelpp & 0.01 & 0.12 & 0.30 & 1023 & 0.05 & 6709 & 0.85\\
        & BoxEL     & 0.00 & 0.01 & 0.05 & 5374 & 0.00 & 13413 & 0.71        \\
        & ELBE     & 0.01   & 0.10          & 0.24          & 1156 & 0.04 & 5657          & 0.88          \\
        & \boxsqel & \textbf{0.03} & \textbf{0.17} & \textbf{0.58} & \textbf{58} & \textbf{0.08} & \textbf{2686} & \textbf{0.94} \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF2}}      & ELEm     & 0.12   & 0.49          & 0.63          & 11   & 0.24 & 4508          & 0.90          \\
        & \emelpp & 0.11 & 0.44 & 0.55 & 23 & 0.21 & 5169 & 0.89\\
        & BoxEL & 0.00 & 0.00 & 0.00 & 22882 & 0.00 & 23007 & 0.50\\
        & ELBE     & 0.01   & 0.05          & 0.09          & 6456 & 0.02 & 9421          & 0.80          \\
        & \boxsqel & \textbf{0.18} & \textbf{0.58} & \textbf{0.75} & \textbf{6}  & \textbf{0.31} & \textbf{2104} & \textbf{0.95} \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF3}} & ELEm     & \textbf{0.06} & \textbf{0.40} & 0.52 & \textbf{54} & \textbf{0.15} & 6292          & 0.86          \\
        & \emelpp & 0.05 & 0.39 & 0.48 & 210 & \textbf{0.15} & 7788 & 0.83\\
        & BoxEL & 0.00 & 0.00 & 0.00 & 17027 & 0.00 & 18947 & 0.59\\
        & ELBE     & 0.02   & 0.15          & 0.30          & 959  & 0.07 & 7131          & 0.84          \\
        & \boxsqel & 0.00   & 0.18          & \textbf{0.53}          & 79   & 0.05 & \textbf{5042} & \textbf{0.89} \\ \midrule
        \multirow{5}{*}{\rotatebox{90}{NF4}} & ELEm     & 0.01 & 0.49 & 0.60          & \textbf{12} & 0.12 & 6272          & 0.86          \\
        & \emelpp & 0.01 & 0.49 & 0.58 & \textbf{12} & 0.13 & 6442 & 0.86\\
        & BoxEL & \textbf{0.09} & \textbf{0.54} & 0.54 & 2215 & \textbf{0.28} & 9673 & 0.79\\
        & ELBE     & 0.00   & 0.07          & 0.12          & 9049 & 0.02 & 12868         & 0.72          \\
        & \boxsqel & 0.00   & 0.37          & \textbf{0.64} & 20   & 0.08 & \textbf{4989} & \textbf{0.89} \\ \bottomrule
    \end{tabular}%
\end{table*}

==> tables/hyper_ppi.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}
\centering
\caption{Hyperparameters for the PPI prediction task.}
\label{tab:hyper_ppi}
\begin{tabular}{@{}lcccccc@{}}
\toprule
      & $n$ & $\gamma$ & lr        & $\delta$ & $\omega$ & $\lambda$ \\ \midrule
Yeast & 200 & 0.02     & $1\times 10^{-2}$ & 2.5        & 4        & 0.2      \\ \midrule
Human & 200 & 0.005     & $5\times 10^{-2}$ & 3.5        & 5        & 0.3      \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/hyper_reasoning.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\centering
\caption{Hyperparameters for the deductive reasoning task.}
\label{tab:hyper_reasoning}
\begin{tabular}{@{}llcccccc@{}}
\toprule
                                         & Model    & $n$ & $\gamma$ & lr        & $\delta$ & $\omega$ & $\lambda$ \\ \midrule
\multirow{5}{*}{\rotatebox{90}{GALEN}}   & ELEm     & 200 & 0        & $5\times 10^{-4}$ & --       & --       & --        \\
                                         & \emelpp  & 200 & 0        & $5\times 10^{-4}$ & --       & --       & --        \\
                                         & BoxEL  & 25 & --        & $5\times 10^{-3}$ & --       & --       & --        \\
                                         & ELBE     & 200 & 0.15      & $1\times 10^{-2}$ & --       & --       & --        \\
                                         & \boxsqel & 200 & 0.05     & $5\times 10^{-3}$ & 1        & 2        & 0         \\ \midrule
\multirow{5}{*}{\rotatebox{90}{GO}}      & ELEm     & 200 & 0.1      & $1\times 10^{-3}$ & --       & --       & --        \\
                                         & \emelpp  & 200 & 0.1      & $1\times 10^{-3}$ & --       & --       & --        \\
                                         & BoxEL  & 25 & --        & $1\times 10^{-3}$ & --       & --       & --        \\
                                         & ELBE     & 200 & 0.05     & $5\times 10^{-3}$ & --       & --       & --        \\
                                         & \boxsqel & 200 & 0.05     & $5\times 10^{-3}$ & 3        & 3        & 0.05      \\ \midrule
\multirow{5}{*}{\rotatebox{90}{Anatomy}} & ELEm     & 200 & 0.05     & $5\times 10^{-4}$ & --       & --       & --        \\
                                         & \emelpp  & 200 & 0.05     & $5\times 10^{-4}$ & --       & --       & --        \\
                                         & BoxEL  & 25 & --        & $1\times 10^{-3}$ & --       & --       & --        \\
                                         & ELBE     & 200 & 0.05     & $5\times 10^{-3}$ & --       & --       & --        \\
                                         & \boxsqel & 200 & 0.05     & $1\times 10^{-3}$ & 2        & 2        & 0.05      \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/inferences.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}
    \centering
    \begin{tabular}{@{}lrrrrrrr@{}}
        \toprule
        Dataset & Hits@1 & Hits@10 & Hits@100 & Med & MRR  & MR   & AUC  \\ \midrule
        GALEN   & 0.01   & 0.09    & 0.25     & 871 & 0.04 & 2715 & 0.88 \\
        GO      & 0.00   & 0.10    & 0.47     & 118 & 0.04 & 1978 & 0.96 \\
        ANATOMY & 0.00   & 0.09    & 0.33     & 324 & 0.03 & 1594 & 0.99 \\ \bottomrule
    \end{tabular}
    \caption{galen}
    \label{tab:galen}
\end{table}

==> tables/test.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
    \centering
    \begin{tabular}{@{}llrrrrrr@{}}
        \toprule
        Dataset                           & Model           & Hits@1        & Hits@10       & Hits@100      & Med          & MR            & AUC           \\ \midrule
        \multirow{4}{*}{\textsf{GALEN}}   & ELEm            & 0.01          & 0.08          & 0.15          & 6658         & 8321          & 0.64          \\
        & EmEL\texttt{++} & 0.02          & 0.11          & 0.17          & 6623         & 8407          & 0.65          \\
        & BoxEL           & --            & 0.12          & 0.23          & --           & 2922          & 0.89          \\
        & ELBE & \textbf{0.04} & \textbf{0.27} & \textbf{0.52} & \textbf{84}  & \textbf{2104} & \textbf{0.91} \\ \midrule
        \multirow{4}{*}{\textsf{GO}}      & ELEm            & 0.01          & 0.09          & 0.23          & 4302         & 13719         & 0.73          \\
        & EmEL\texttt{++} & 0.01          & 0.10          & 0.24          & 2908         & 11050         & 0.78          \\
        & BoxEL           & --            & 0.09          & 0.24          & --           & 8010          & 0.83          \\
        & ELBE & \textbf{0.02} & \textbf{0.12} & \textbf{0.27} & \textbf{865} & \textbf{5458} & \textbf{0.88} \\ \midrule
        \multirow{4}{*}{\textsf{ANATOMY}} & ELEm            & 0.04          & 0.19          & 0.41          & 640          & 28564         & 0.73          \\
        & EmEL\texttt{++} & 0.04          & 0.18          & 0.40          & 381          & 24421         & 0.76          \\
        & BoxEL           & --            & 0.19          & 0.43          & --           & \textbf{8688} & \textbf{0.92} \\
        & ELBE            & \textbf{0.05} & \textbf{0.20} & \textbf{0.46} & \textbf{159} & 12850         &               \\ \bottomrule
    \end{tabular}
    \caption{Test caption}
    \label{tab:test}
\end{table}
